The COS Absorption Survey of Baryon Harbors: The Galaxy Database and Cross-Correlation Analysis of OVI Systems

We describe the survey for galaxies in the fields surrounding 9 sightlines to far-UV bright, z~1 quasars that define the COS Absorption Survey of Baryon Harbors (CASBaH) program. The photometry and spectroscopy that comprise the dataset come from a mixture of public surveys (SDSS, DECaLS) and our dedicated efforts on private facilities (Keck, MMT, LBT). We report the redshifts and stellar masses for 5902 galaxies within ~10 comoving-Mpc (cMpc) of the sightlines with a median of z=0.28 and M_* ~ 10^(10.1) Msun. This dataset, publicly available as the CASBaH specDB, forms the basis of several recent and ongoing CASBaH analyses. Here, we perform a clustering analysis of the galaxy sample with itself (auto-correlation) and against the set of OVI absorption systems (cross-correlation) discovered in the CASBaH quasar spectra with column densities N(O^+5) >= 10^(13.5)/cm^2. For each, we describe the measured clustering signal with a power-law correlation function xi(r) = (r/r_0)^(-gamma) and find that (r_0,gamma) = (5.48 +/- 0.07 h_100^-1 Mpc, 1.33 +/- 0.04) for the auto-correlation and (6.00 +/- 1 h^-1 Mpc, 1.25 +/- 0.18) for galaxy-OVI cross-correlation. We further estimate a bias factor of b_gg = 1.3 +/- 0.1 from the galaxy-galaxy auto-correlation indicating the galaxies are hosted by halos with mass M_halo ~ 10^(12.1 +/- 0.05) Msun. Finally, we estimate an OVI-galaxy bias factor b_OVI = 1.0 +/- 0.1 from the cross-correlation which is consistent with OVI absorbers being hosted by dark matter halos with typical mass M_halo ~ 10^(11) Msun. Future works with upcoming datasets (e.g., CGM^2) will improve upon these results and will assess whether any of the detected OVI arises in the intergalactic medium.

==> tab_sub_targets.tex <==
\begin{deluxetable*}{lccccc}
\tablewidth{0pc}
\tablecaption{CASBaH Targeted Candidate Galaxies\label{tab:targets}}
\tabletypesize{\small}
\tablehead{\colhead{Field} & \colhead{RA} 
& \colhead{DEC} & \colhead{$m_{target}$}  & \colhead{Filter} 
& \colhead{Instr.} 
} 
\startdata 
PG1630+377&248.08537 &37.40200 &23.65 &R &DEIMOS \\ 
PG1630+377&247.91914 &37.40197 &23.65 &R &DEIMOS \\ 
PG1630+377&248.09161 &37.40208 &23.49 &R &DEIMOS \\ 
PG1630+377&247.92538 &37.40207 &23.49 &R &DEIMOS \\ 
PG1630+377&248.00459 &37.40681 &16.24 &R &DEIMOS \\ 
PG1630+377&248.00576 &37.42155 &22.57 &R &DEIMOS \\ 
PG1630+377&248.15386 &37.42810 &25.00 &R &DEIMOS \\ 
PG1630+377&247.90408 &37.42827 &24.69 &R &DEIMOS \\ 
PG1630+377&247.94370 &37.42849 &24.51 &R &DEIMOS \\ 
PG1630+377&247.86827 &37.42845 &23.83 &R &DEIMOS \\ 
\enddata 
\end{deluxetable*} 

